Differentiable Invariant Causal Discovery

Learning causal structure from observational data is a fundamental challenge in machine learning. However, the majority of commonly used differentiable causal discovery methods are non-identifiable, turning this problem into a continuous optimization task prone to data biases. In many real-life situations, data is collected from different environments, in which the functional relations remain consistent across environments, while the distribution of additive noises may vary. This paper proposes Differentiable Invariant Causal Discovery (DICD), utilizing the multi-environment information based on a differentiable framework to avoid learning spurious edges and wrong causal directions. Specifically, DICD aims to discover the environment-invariant causation while removing the environment-dependent correlation. We further formulate the constraint that enforces the target structure equation model to maintain optimal across the environments. Theoretical guarantees for the identifiability of proposed DICD are provided under mild conditions with enough environments. Extensive experiments on synthetic and real-world datasets verify that DICD outperforms state-of-the-art causal discovery methods up to 36% in SHD. Our code will be open-sourced.

==> chapters/0_abstract.tex <==
\begin{abstract}
% Background: CD is a fundamental problem
Learning causal structure from observational data is a fundamental challenge in machine learning. 
% Existing methods and their limitations
However, the majority of commonly used differentiable causal discovery methods are non-identifiable, turning this problem into a continuous optimization task prone to data biases. 
In many real-life situations, data is collected from different environments, in which the functional relations remain consistent across environments, while the distribution of additive noises may vary.
This paper proposes \underline{D}ifferentiable \underline{I}nvariant \underline{C}ausal \underline{D}iscovery (\textbf{DICD}), utilizing the multi-environment information based on a differentiable framework to avoid learning wrong causal directions.
Specifically, DICD aims to discover the environment-invariant causation while removing the environment-dependent correlation.
We further formulate the constraint that enforces the target structure equation model to maintain optimal across the environments.
Theoretical guarantees for the identifiability of proposed DICD are provided under mild conditions with enough environments.
Extensive experiments on synthetic and real-world datasets verify that DICD outperforms state-of-the-art causal discovery methods up to 36\% in SHD. Our code is open-sourced at \url{https://anonymous.4open.science/r/DICD-9271/}.
\end{abstract}
